On Training Robust PDF Malware Classifiers

Although state-of-the-art PDF malware classifiers can be trained with almost perfect test accuracy (99%) and extremely low false positive rate (under 0.1%), it has been shown that even a simple adversary can evade them. A practically useful malware classifier must be robust against evasion attacks. However, achieving such robustness is an extremely challenging task. In this paper, we take the first steps towards training robust PDF malware classifiers with verifiable robustness properties. For instance, a robustness property can enforce that no matter how many pages from benign documents are inserted into a PDF malware, the classifier must still classify it as malicious. We demonstrate how the worst-case behavior of a malware classifier with respect to specific robustness properties can be formally verified. Furthermore, we find that training classifiers that satisfy formally verified robustness properties can increase the evasion cost of unbounded (i.e., not bounded by the robustness properties) attackers by eliminating simple evasion attacks. Specifically, we propose a new distance metric that operates on the PDF tree structure and specify two classes of robustness properties including subtree insertions and deletions. We utilize state-of-the-art verifiably robust training method to build robust PDF malware classifiers. Our results show that, we can achieve 92.27% average verified robust accuracy over three properties, while maintaining 99.74% accuracy and 0.56% false positive rate. With simple robustness properties, our robust model maintains 7% higher robust accuracy than all the baseline models against unrestricted whitebox attacks. Moreover, the state-of-the-art and new adaptive evolutionary attackers need up to 10 times larger $L_0$ feature distance and 21 times more PDF basic mutations (e.g., inserting and deleting objects) to evade our robust model than the baselines.

==> futurework.tex <==
\section{Future Work}

Design a stronger attack to evaluate this?

Generalization to newer unseen PDF malware.

Extracting exploit and robustness specifications from newer PDF malware automatically.

Generalization of verifiably robust training.

Are robustness properties specific to features and the model?

Compose new robustness properties.

What about cost for whitebox attackers.


What about other models (e.g. SVM)?


==> response.tex <==
\section{Revision Letter}


We greatly appreciate the insightful comments from the reviewers. We have redone the evaluation for the paper, with major changes summarized below.

\begin{enumerate}
\item \textbf{Training and Threat Model:} We have improved our verifiably robust training implementation, to mix train different properties at the mini-batch level (Section 3.2 and 4.1.4), and retrained all the models. We have updated our results based on compact hidost feature~\cite{vsrndic2013detection, hidost_feat} extraction (Section 4.1.1). We added a new robustness property E, that captures insertion-only attack up to the entire feature space.
\item \textbf{New Baseline Models:} We have compared 7 verifiably robust models against 12 baselines in total. As suggested by reviewers, the baselines include regularly trained neural network, adversarially robust trained models, ensemble models and monotonic classifiers (Table 4). We described these models in Section 4.1.3 and evaluated their VRA in Section 4.2.
\item \textbf{Restricted ERA Evaluation:} We added restricted ERA evaluation that is consistent with VRA (Section 4.3). For example, to evaluate robustness property A, the restricted gradient attacker first chooses a subtree, then deletes features guided by gradient until an evasion instance is found, or the entire subtree is deleted. If any of the subtree choices succeeds, the restricted attack succeeds. Since VRA overapproximates attacker’s actions within the bounded property, VRA is the lower bound for the corresponding ERA (Table 4, 5, and 7).
\item \textbf{Unrestricted Whitebox Attacks:} We evaluated our verifiably robust models against unrestricted whitebox attacks compared to neural network baselines and monotonic classifiers. For neural network models (including verifiably robust models), we ran unrestricted gradient attack with both insertion and deletion, on 3416 test PDF malware, until all evasion instances are found or 200,000 iterations (Section 4.3). For monotonic classifiers, we ran the unrestricted Mixed Integer Linear Program (MILP) attack, until all evasion instances are found (Section 4.4). The Robust A+B model maintains 7\% higher ERA than all baselines after 200,000 iterations. Lastly, we converted evasive feature vectors found by the gradient and MILP attacks to real PDFs (Section 4.3.2, 4.4.1 and Appendix A.4). If we enforce that the corresponding PDFs are malicious, the average ERA of NN models increased to 94.25\%, and the average ERA of monotonic classifiers increased to 100\%, since the feature-space attacks often break the semantics of PDF.
\item \textbf{Unrestricted Blackbox Attacks:} We evaluated how much our verifiably robust models can increase the ERA, $L_0$ distance and mutation trace length for unrestricted blackbox attackers, compared to the strongest baseline models. Against the reverse mimicry attack, our Robust A+B+E model achieves the highest ERA, 50.8\% (Section 4.6). For evolutionary attacks, we go through the list of randomly scheduled PDFs by rounds of attacks,
until all of them are evaded. The state-of-the-art evolutionary attacker needs up to 3.6 times larger $L_0$ distance, and 21 times more mutations to evade our Robust A+B model than the best baselines (Section 4.5 and Appendix A.6). Moreover, we implemented new adaptive strategies, including move exploit mutation to target property E, and scatter insertion and deletion under different subtrees to target property A and B. The adaptive evolutionary attack needs 10 times larger $L_0$ distance, and 3.7 times more mutations to evade our Robust A+B model than the monotonic classifier (Section 4.7 and Appendix A.6).
\item \textbf{Others:} We motivated the specification of the robustness properties (Section 3.1.1), and formally defined the subtree distance (Section 3.1.2). We added precision and recall of the models in Table 7. We clarified writing issues according to the reviewer’s comments. We will release a set of robust models, and we are working on open sourcing our implementation.
\end{enumerate}
